Privacy Preserving Driving Style Recognition

In order to better manage the premiums and encourage safe driving, many commercial insurance companies (e.g., Geico, Progressive) are providing options for their customers to install sensors on their vehicles which collect individual vehicle's traveling data. The driver's insurance is linked to his/her driving behavior. At the other end, through analyzing the historical traveling data from a large number of vehicles, the insurance company could build a classifier to predict a new driver's driving style: aggressive or defensive. However, collection of such vehicle traveling data explicitly breaches the drivers' personal privacy. To tackle such privacy concerns, this paper presents a privacy-preserving driving style recognition technique to securely predict aggressive and defensive drivers for the insurance company without compromising the privacy of all the participating parties. The insurance company cannot learn any private information from the vehicles, and vice-versa. Finally, the effectiveness and efficiency of the privacy-preserving driving style recognition technique are validated with experimental results.

==> pro.tex <==





\comment{

\subsection{Cryptographic Building Blocks}\label{sec:buildb}

The basic cryptographic building block is the Secure Sum (for information gain).  Using this method for securie multi-party communication,
the computational transaction is made entirely in ciphertext, protecting both parties from unintentional information sharing.  Since both
parties are sharing only ciphertext, the risk of information spillage is very low when the semi-honest model is assumed.
}
